Improving Policy Gradient by Exploring Under-appreciated Rewards

This paper presents a novel form of policy gradient for model-free reinforcement learning (RL) with improved exploration properties. Current policy-based methods use entropy regularization to encourage undirected exploration of the reward landscape, which is ineffective in high dimensional spaces with sparse rewards. We propose a more directed exploration strategy that promotes exploration of under-appreciated reward regions. An action sequence is considered under-appreciated if its log-probability under the current policy under-estimates its resulting reward. The proposed exploration strategy is easy to implement, requiring small modifications to an implementation of the REINFORCE algorithm. We evaluate the approach on a set of algorithmic tasks that have long challenged RL methods. Our approach reduces hyper-parameter sensitivity and demonstrates significant improvements over baseline methods. Our algorithm successfully solves a benchmark multi-digit addition task and generalizes to long sequences. This is, to our knowledge, the first time that a pure RL method has solved addition using only reward feedback.

==> expts.tex <==

\iffalse
\begin{table}[t]
\caption{Results}
\label{gym-results}
\begin{center}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|}
\cline{2-11}
 & \multicolumn{8}{c|}{\bf \pg} & \multicolumn{2}{c|}{\bf \rml} \\ \cline{2-11}
 & \multicolumn{2}{c|}{$\tau=0.0$} & \multicolumn{2}{c|}{$\tau=0.005$} & \multicolumn{2}{c|}{$\tau=0.01$} & 
   \multicolumn{2}{c|}{$\tau=0.1$} & \multicolumn{2}{c|}{$\tau=0.1$} \\ \hline
\multicolumn{1}{|l|}{\bf Copy} 		&  85.0 & 5 & 88.3 & 5 & {\bf 90.0} & {\bf 5} & 3.3 & 1 & 75.0 & 5 \\ \hline
\multicolumn{1}{|l|}{\bf DuplicatedInput} 	& 68.3 & 5 & 73.3 & 5 & 73.3 & 5 & 0.0 & 0 & {\bf 100.0} & {\bf 5} \\ \hline
\multicolumn{1}{|l|}{\bf RepeatCopy} 	& 0.0 & 0 & 0.0 & 0 & 11.6 & 3 & 0.0 & 0 & {\bf 18.3} & {\bf 4} \\ \hline
\multicolumn{1}{|l|}{\bf Reverse} 		& 0.0 & 0 & 0.0 & 0 & 3.3 & 1 & 10.0 & 2 & {\bf 16.6} & {\bf 4} \\ \hline
\multicolumn{1}{|l|}{\bf ReversedAddition} 	& 0.0 & 0 & 0.0 & 0 & 1.6 & 1 & 0.0 & 0 & {\bf 30.0} & {\bf 5} \\ \hline
\end{tabular}
\end{center}
\end{table}
\fi

